How a well-adapted immune system is organized

The repertoire of lymphocyte receptors in the adaptive immune system protects organisms from diverse pathogens. A well-adapted repertoire should be tuned to the pathogenic environment to reduce the cost of infections. We develop a general framework for predicting the optimal repertoire that minimizes the cost of infections contracted from a given distribution of pathogens. The theory predicts that the immune system will have more receptors for rare antigens than expected from the frequency of encounters; individuals exposed to the same infections will have sparse repertoires that are largely different, but nevertheless exploit cross-reactivity to provide the same coverage of antigens; and the optimal repertoires can be reached via the dynamics of competitive binding of antigens by receptors, and selective amplification of stimulated receptors. Our results follow from a tension between the statistics of pathogen detection, which favor a broader receptor distribution, and the effects of cross-reactivity, which tend to concentrate the optimal repertoire onto a few highly abundant clones. Our predictions can be tested in high throughput surveys of receptor and pathogen diversity.

==> sections/Old/res2.tex <==
% Punchline 2
% - cross-reactivity limits optimal diversity
% - if cross-reactivity is large compared to pathogen distribution fluctuations --> Delta distribution

\subsection{Cross-reactivity dramatically limits optimal repertoire diversity}
\label{sec:res2}

\begin{figure}
    \centering
    \includegraphics{fig/crossreactivityanalytical}
    \caption{
        {\TM Optimal receptor distribution and cost for protecting against
a one-dimensional Gaussian antigenic landscape $Q(a)$ of variance $\sigma_Q^2$,}
%an analytically solvable example,
as a function of the cross-reactivity width $\sigma$.
{\TM As the $\sigma$ increases, the optimal distribution $P^*(r)$ becomes narrower and narrower (left and middle insets), until it concentrates entirely onto a single point, for $\sigma\geq \sqrt{2}\sigma_Q$ (right inset).
        The minimal cost (normalized by $\sigma$ for a comparison at constant recognition capability) 
is constant below the transition point, but increases with $\sigma$ past it.
%        The antigen distribution $Q(a)$ is Gaussian.
Here the cross-reactivity kernel, which quantifies the affinity between receptor $r$ and antigen $a$ as a function of their distance in shape space, is assumed to have a Gaussian form:
        %We assume furthermore that cross-reactivity can be described by a Gaussian kernel
        $f(r-a) = \exp[-(r-a)^2 / 2\sigma^2]$,
       and the cost function is linear in the effective recognition time, $F(m) = m$.}
% first remains constant, before starting to increase for $\sigma>\sqrt{2}\sigma_Q$.
%        Insets show the pathogen distribution $Q(a)$ and the optimal receptor distribution $P^\star(r)$ for three choices of $\sigma/\sigma_Q$ on both sides of the transition. The optimal receptor distribution becomes narrower as the cross-reactivity width is increased, until it becomes a Dirac delta function at the transition.
}
    \label{fig:crossreactivityanalytical}
\end{figure}


\begin{figure}
    \centering
    \includegraphics{fig/crossreactivity}
    \caption{Cross-reactivity plays an important role in shaping the optimal repertoire, often leading to highly peaked repertoires.        
\TM
%        (A)-(B) Results from numerical optimization for random antigen landscapes generated according to $Q \propto \ln \mathcal{N}(\kappa)$.
        The optimal receptor distribution $P^*(r)$ is represented for (A) one- and (B) two-dimensional random environments.
{\TM
Despite being peaked, the optimal distribution of receptors covers the antigenic space fairly uniformly, as shown by its coverage by the receptors, $\tilde P^*(a)=\int dr f(a-r)P^*(r)$, represented in the one-dimensional case (A).}
As in Fig.~\ref{fig:crossreactivityanalytical}, the cross-reactivity kernel is assumed to be Gaussian,
        %$f(r-p) = \exp\((-\frac{|r-p|^2}{2\sigma^2}\))$
        $f(r-p) = \exp[-(r-p)^2 / 2\sigma^2]$,
        and the effective cost function to be linear, $F(m) = m$.
        {\TM The antigenic landscape $Q(a)$ is generated randomly as the exponential of a Gaussian white noise of amplitude $\kappa=1$. The numerical problem was solved with a discretization step of $0.1\sigma$.}
%        (A) Exemplary cutout of an optimal receptor distribution.
 %       A one dimensional receptor -- antigen space with periodic boundary conditions is used.
%        The problem is discretized on a $10\sigma$ grid with a discretization spacing of $0.1\sigma$. 
%        Due to cross-reactivity the space is still covered fairly uniformly by this collection of peaks. 
%as shown by the coverage $\tilde P^\star$.
        %$\kappa = 1$ is used.
        %(c) Mean spacing between peaks in the optimal receptor distributions increases with $\sigma$.
        %The slope of the linear regression line is $\sim 1.6$.
%        (B) Two dimensional receptor -- antigen space with periodic boundary conditions.
%        The problem is discretized on a $30\sigma \times 30\sigma$ grid with a discretization spacing of $0.1\sigma$.
 %       (C) Exemplary cutout of an optimal receptor distribution for $\kappa = 1$.        
    }
    \label{fig:crossreactivity}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics{fig/crossreactivityanalysis}
    \caption{
{\TM Structural analysis of the tiling pattern formed by the peaks of the optimal distribution of receptors $P^*(r)$, in two dimensions (see also Fig.~\ref{fig:crossreactivity}B).
        (A) The radial distribution function of $P^*(r)$ (defined by Eq.~\ref{eq:rdf}) shows a exclusion zone around each peak, followed by oscillations characteristic of a local tiling pattern.
        (B) Normalized power spectral density $S(q)$ of $P^*(r)$ (defined by Eq.~\ref{eq:sq}) for different values of the parameter $\kappa$ quantifying the heterogeneity of the antigenic lanscape. The high suppression of fluctuations at large scales (small $q$) indicates that the pattern has very little fluctuations in the number of receptors used to cover equal surface areas.
        (C) The power spectral density of $P^*(r)$, now normalized by $\kappa^2$, shows that the fluctuations at large scale are entirely attributable to those of the antigenic environment, and scale with them, as demonstrated by the data collapse.}
        The results in (A) and (B) are averaged over 10 independent runs to reduce stochastic fluctuations.
%        \todo{The values here do not correspond to those used in the simulations. Need to do the simulations.}
    }
    \label{fig:crossreactivityanalysis}
\end{figure*}

In the absence of cross-reactivity, the immune system must have receptors against every possible antigen for full protection, {\TM as discussed in the previous section. Cross-reactivity, the ability of receptors to bind to a variety of different antigens, should in principle allow for a more parsimonious use of receptors to cover the whole range of possible threats. Indeed we will show that, in many cases, the optimal solution concentrates its resources on a few receptors, which together tile the antigenic space.}
%In the presence of cross-reactivity this is no longer the case.

%We now explore how to optimally introduce receptor cross-reactivity to focus resources on where they are most needed.

Following Perelson and Oster \cite{oster-1979},  we can think of receptors and antigens as points in a common highly dimensional {\it shape space}, whose coordinates can be associated with unspecified physicochemical properties. For simplicity we assume %that the antigen and receptor space can be identified with each other and that 
the cross-reactivity only depends on the relative position of receptor and antigen in shape space $f_{r,a} = f(r-a)$,  {\TM where $f$ is a decreasing function of the distance between $a$ and $r$.}
Short distances in shape space correspond {\TM to a good fit between the two molecules, leading to} strong recognition, while large distances translate into weak interactions and poor recognition.%{\color{red} [TM- we haven't said what space we're in, so this is a big ambiguous. from here on we need to introduce the notion of shape space and cite Perelson et al.]}

In order to build some intuition about the problem, we first consider an analytically solvable example, in which the space of receptors and antigens is described by a single continuous number.
{\TM We assume that the antigen distribution is Gaussian of variance $\sigma_Q^2$, and that the  cross-reactivity function also has a Gaussian form: $f(x)=\exp(-x^2/2\sigma^2)$, where $\sigma$ is the cross-reactivity width, {\em i.e.} the typical distance within which a receptor and an antigen interact.
The total recognition capability, $\int dx f(x)=\sqrt{2\pi}\sigma$, increases linearly with $\sigma$. Therefore, to make fair comparisons between different values of $\sigma$, we will normalize the overall cost by $\sigma$.}
%We compare costs at constant total capacity of recognition, i.e. we normalize $f_{r,a}$.

For costs {\TM of the form} $F(m) = m^\alpha$, we can derive the optimal receptor distributions and costs analytically (see App.~\ref{app:gaussian}). 
The results show two different regimes {\TM depending on the value of the cross-reactivity width $\sigma$}, as illustrated in Fig.~\ref{fig:crossreactivityanalytical}.
{\TM The optimal normalized cost is constant for narrow cross-reactivities (low $\sigma$), and starts to increase past a critical value $\sigma_c$.
These two regimes correspond to qualitatively different optimal receptor distributions:
a Gaussian distribution of variance $(1+\alpha)\sigma_Q^2 - \sigma^2$ below the threshold, and a Dirac delta distribution above it.
The $1+\alpha$ factor broadens the optimal receptor distribution with respect to the antigen distribution, in accord with the discussion of the previous section, while
cross-reactivity has the opposite effect, leading to a more concentrated distribution.
At the critical value $\sigma_c = \sigma_Q\sqrt{1+\alpha} $, the optimal receptor distribution becomes a Dirac delta function, which it remains for $\sigma>\sigma_c$.
%Since no further narrowing is possible, the distribution remains unchanged as $\sigma$ is increased beyond $\sigma_c$.
Above the critical $\sigma_c$, the high cross-reactivity means that the system is wasting resources far away from the center of the pathogen distribution, where little antigen threat is present, resulting in an increase of the cost.}
%the amount of recognition capacity that is unused in the tails of the antigen distribution increases, which explains the increase in the cost function for $\sigma > \sigma_c$.

{\TM How generic is this phenomenon by which the distribution clusters into peaks? To investigate this question we turn to numerical optimisation.}
%To generalize the result that cross-reactivity %limits local receptor diversity, leading to strongly peaked distributions, holds more generally, 
%leads to strongly peaked receptor distributions we turn to numerical optimization. %{\color{red} [TM- rewrite sentence]}
{\TM For concreteness we consider random pathogen environments in one or two dimensions (modeled by a lognormal white noise distribution of antigens) and assume a linear cost function $F(m)=m$.
For the purpose of the numerics the space is finite and discretized. The optimization problem is solved by an accelerated gradient projection algorithm (App.~\ref{app:numerics}).}
%For concreteness, we choose a lognormal white noise distribution of antigens \todo{biological motivation} and assume a linear cost $F(m) = m$, but we do not expect these assumptions to qualitatively change our conclusions. \todo{Andreas says: expand in appendix}.

%Generate random numbers from $\ln \mathcal{N}(\kappa) = exp(\kappa Z)$, where $Z$ is a standard normal random variable. Then normalize the distribution.
%\todo{expand}


The numerical results lead to strongly peaked distributions in both one and two dimensions (Fig.~\ref{fig:crossreactivity}A,B), generalizing the observation that cross-reactivity severely limits local receptor diversity.
{\TM Compared to the Gaussian case discussed earlier, where the antigen distribution only had one scale $\sigma_Q$, here the random antigen distribution includes all possible scales. By analogy with the Gaussian case, we expect the smallest scales to lead Dirac delta peaks. The observed peaks are evenly spaced, with an inter-peak distance of the same order as the cross-reactivity width $\sigma$.}
%{\TM [don't get this argument]} In the Gaussian case we saw that the variance of the receptor distributions depended on the variance of the antigen distribution relative to the cross-reactivity. In the numerical result, the antigen distribution (blue line in Fig.~\ref{fig:crossreactivity}A) has multiple scales and we {\TM could} expect the receptor distribution to exhibit peaks mirroring the antigen distribution.  %Although the random antigen distribution used in the numerical calculation has features at many scales, whereas the Gaussian distribution in the analytical calculation has only one characteristic scales, both results exhibit a  strongly peaked receptor distributions. {\color{red} [TM- twice the same sentence?]}
%The spacing of the peaks in the case of the random antigen distribution is similar to the critical cross-reactivity $\sigma_c=\sigma{2}\sigma$ {\TM discussed earlier}.
%{\TM [TM- does not seem true in 1D]}
Additionally, the peaks of the receptor distribution approach the limit of Dirac delta functions as the numerical discretization step tends to zero, {\TM suggesting that the true solution is a weighted sum of Dirac deltas} (see Fig.~\ref{fig:dirac}).

The position of the peaks is not random but shows a {\it tiled} structure, which is best seen in the 2D example (Fig. \ref{fig:crossreactivity}B).
To analyze this structure quantitatively, we use a {\TM measure commonly used in condensed matter physics to describe the arrangement of molecules in liquids, cristals, glass or packing of spheres ---\,the radial distribution function, which measures correlation between peak positions \cite{ChaikinLubensky}:}
\begin{equation} \label{eq:rdf}
    g(r) = \av{P(r_1) P(r_2)}_{|r_1 - r_2|=r}
\end{equation}
{\TM where $|r_1-r_2|$ is the distance between $r_1$ and $r_2$.}
Fig.~\ref{fig:crossreactivityanalysis}A represents $g(r)$ for the 2D tiling. {\TM The initial drop at small $r$ indicates that}
there is little chance to find two peaks close to each other, {\TM meaning that peaks tend to repel each other}.
This exclusion is a sensible way to distribute resources, as it tends to limit redundant protection of the same region.
The range of distances over which this effective repulsion occurs is of the order of $\sigma$, in line with this argument. {\TM This allows us to draw an analogy with the problem of sphere packing. When brought to very high densities, hard spheres must cover as much space as possible while maintaining an exclusion zone with other spheres. Our optimisation problem solves a similar problem. When the density becomes very high, packed spheres organise into a disordered tiling pattern, evidenced by damped oscillations in $g(r)$, similar to what we observe. Such a tiling ensures a regular distribution of receptors and a uniform coverage of the antigenic space.
}

{\TM To quantify how regular the tiling is}, we calculated {\TM the normalized power spectral density} of the 2D pattern. 
%{\TM Assuming that $P(r)$ can be written as a sum of $n$ Dirac deltas, $P(r)=\sum_{i=1}^n p_i\delta(r-r_i)$, 
{\TM We define this spectral density as:}
%\begin{equation} \label{eq:sq}
%    S(q) = \av{\frac{|FT P(r)|^2}{\int \ud r P(r)^2}},
%\end{equation}
\begin{equation}\label{eq:sq}
S(q)=\frac{\sum_{r,r'} P_rP_{r'} e^{{\rm i} q(r-r')}}{\sum_r P_r^2},
\end{equation}
{\TM where $q$  is the wave vector. The normalization is chosen such that, when $P_r$ is made of peaks of uniform heights, $S(q)$ coincides with the {\em structure factor} familiar in condensed matter physics, which satisfies
$S(q \rightarrow \infty) = 1$. Fig.~\ref{fig:crossreactivityanalysis}B shows $S(q)$ averaged over many realizations, and over all directions of $q$ so that it only depends on its modulus $|q|$.}
{\TM As expected}, $S(q)$ approaches 1 for large $q$, reflecting the randomness of the precise position of the peaks locally. {\TM (The small departure from $1$ is attributable to the form factor of the peaks, which results from the discretization procedure.)}
$S(q)$ is very low for small $q$, indicating that fluctuations in the number of receptors per surface area are small at large scales. {\TM In other words, the number of receptors contained in a large given area of the shape space is very reproducible. This phenomenon, called {\em hyperuniforminity} in condensed matter \cite{stillinger-2003}, is linked to the incompressibility of the material, and characteristic of jammed packings \cite{Donev:2005p13220,Berthier:2011p13219}.
}
%The structure factor 

%This  behaviour is similar to that predicted for a solid.
{\TM This hyperuniforminity} provides insight into how space is covered {\TM in the optimal solution}:
at large scales (small $q$) the fluctuations in the number of receptors should be suppressed to cover the space more or less uniformly, whereas 
the small scale fluctuations (large $q$) get smoothed out by cross-reactivity and can be tolerated.
{\TM At small $q$, the fluctuations in the optimal receptor distribution are entirely driven by those of the antigenic landscape, modulated by the cross-reactivity function $f$. At these large scales, the power spectrum of the receptor distribution is approximately given by:
$|\sum_r P_r e^{\mathrm{i}qr}|^2\sim \kappa^2 \exp[(q\sigma)^2/2]/4$, where $\kappa$ is magnitude of fluctuations in $Q$, and the exponential term stems from the inverse of the Fourier transform of $f$ (see Appendix). We check this relation by plotting the power spectral density normalized by $\kappa^2$
(Fig.~\ref{fig:crossreactivityanalysis}C), and verify that all curves collapse onto the theoretical prediction $\exp[(q\sigma)^2/2]/4$.
}
%We furthermore see that the fluctuations for small $q$ are purely driven by antigen fluctuations, as seen from the rescaled structure factor that follows exactly the spectral components of the antigen distribution (black line).
%{\color{red} [TM- use the word tiling somewhere?]}
%the fluctuations follows directly the antigen distribution in magnified form (cross-reactivity smoothens!) up to a certain q. {\color{red} ????} 


{\TM 
So far our analysis has focused on particular choices of the antigenic environment (random white noise), and the cross-reactivity kernel $f$ (Gaussian). To test the generality of our results}, we investigated whether strongly peaked repertoires
were also optimal {\TM in other conditions}. We find that the choice of the cross-reactivity function can qualitatively impact the optimal repertoire. As shown in Fig.~\ref{fig:kernels}, changing the cross-reactivity function does not
change the peaked nature of the optimal repertoire, but it does change number and position of the peaks. 
%The antigen distribution we obtain by drawing a number of independent
%random numbers is uncorrelated.
%As antigens mutate, on short timescales the distribution may be correlated, as we have assumed in the analytical example. 
{\TM To account for possible correlations in the distribution of antigens across the effective shape space (reflecting {\em e.g.} phylogenic correlations between pathogens),}
we also generated random correlated antigen distributions by filtering white noise.
In this case we find peaked optimal receptor distributions (Fig. \ref{fig:correlation}), similarly to those described above for the uncorrelated antigen distribution. %, characteristic of long timescales.
%{\color{red} Aleks says $\to$ Appendix: 
%If the Fourier transform of the kernel has zero crossings, we can have
%non-uniform optimal solutions even for completely uniform antigen
%distributions.
%The Gaussian kernel we have considered so far, might be considered
%marginal between kernels with and without zero crossings
%\citep{hernandez-garcia-2007}.
%Consider the family of Kernel functions
%$\exp\((-\frac{1}{2}\((\frac{x}{\sigma}\))^\gamma\))$, which includes
%the Gaussian as a special case for $\gamma = 2$.
%Up to $\gamma = 2$ all such Kernels have positive Fourier transforms,
%whereas for $\gamma > 2$ the Fourier transforms take negative values
%\citep{hernandez-garcia-2007}.}
%As shown in Fig. \ref{fig:kernels} changing of the cross-reactivity function does not change the peaked nature of the optimal repertoire, but it does change number and position of peaks.
{\TM The shape space of receptors and antigens is probably highly dimensional, some authors estimating as many as five effective dimensions \cite{oster-1979}.
Although our analysis is here restricted to two dimensions for computational reasons, previous work on the dimensional dependence of random packing problems in physics allows us to
expect all these results to hold more generally in higher dimensions.}


%{\color{red} add paragraph about how the results do not depend on choice of pathogen correlation functions and different kernel choices with ref to fig in SI/appendix.}

%In exploring the effect of cross-reactivity we have made considerable simplifications.
%A word of caution is thus in order, but making strong assumptions allowed us to derive interesting results and get an intuition for the problem.
%A mathematical argument suggests, that the peakedness of solutions in presence of cross-reactivity holds relatively generally (see App. \ref{app:mathpeaks}), but future work should check this conclusion numerically and also carefully investigate whether the other conclusions also hold more generally.


==> sections/Old/res2_copy.tex <==
% Punchline 2
% - cross-reactivity limits optimal diversity
% - if cross-reactivity is large compared to pathogen distribution fluctuations --> Delta distribution

%\subsection{Cross-reactivity dramatically limits optimal repertoire diversity}
\subsection{{\VB Cross-reactivity dramatically reduces diversity in the optimal repertoire}}
\label{sec:res2}



{\VB By allowing receptors to bind to a variety of  antigens, cross-reactivity should permit the immune system to reduce the number of receptor types required to cover the whole range of possible threats.   Indeed, we will show that given sufficient cross-reactivity, the optimal immune repertoire concentrates all its resources on a few receptors, which together tile antigenic space.}



%{\TM as discussed in the previous section. Cross-reactivity, the ability of receptors to bind to a variety of different antigens, should in principle allow for a more parsimonious use of receptors to cover the whole range of possible threats. Indeed we will show that, in many cases, the optimal solution concentrates its resources on a few receptors, which together tile the antigenic space.}
%In the presence of cross-reactivity this is no longer the case.

%We now explore how to optimally introduce receptor cross-reactivity to focus resources on where they are most needed.

Following Perelson and Oster \cite{oster-1979},  we will think of receptors and antigens as points in a common high dimensional {\it shape space}, whose coordinates are associated to unspecified physicochemical properties. For simplicity,  assume that cross-reactivity only depends on the relative position of receptor and antigen in shape space $f_{r,a} = f(r-a)$,  {\TM where $f$ is a decreasing function of the distance between $a$ and $r$.}
Short distances in shape space correspond {\TM to a good fit between the two molecules, leading to} strong recognition, while large distances translate into weak interactions and poor recognition.%{\color{red} [TM- we haven't said what space we're in, so this is a big ambiguous. from here on we need to introduce the notion of shape space and cite Perelson et al.]}

In order to build  intuitions, we first consider an analytically solvable example.  Let the space of receptors and antigens be described by a single continuous number.
{\VB Assume a Gaussian antigen distribution with variance $\sigma_Q^2$, and Gaussian cross-reactivity $f(x)=\exp(-x^2/2\sigma^2)$, where $\sigma$ sets the typical distance within which a receptor and  antigen interact.
The total recognition capability, $\int dx f(x)=\sqrt{2\pi}\sigma$, increases linearly with $\sigma$. Therefore, to make fair comparisons between different values of $\sigma$, we will normalize the overall cost by $\sigma$.}
%We compare costs at constant total capacity of recognition, i.e. we normalize $f_{r,a}$.

\ifthenelse{\equal{\format}{pnasfigend}}{}{\paneltwo}

{\VB In this setting we can derive the optimal receptor distributions  analytically for costs {\TM of the form} $F(m) = m^\alpha$
(\ifthenelse{\equal{\ispnas}{true}}{see SI, Sec. D3b}{App.~\ref{app:gaussian}}).
For narrow cross-reactivities ($\sigma < \sigma_c =  \sigma_Q\sqrt{1+\alpha}$), the optimal receptor distribution is  Gaussian with variance $(1+\alpha)\sigma_Q^2 - \sigma^2$ (broader than the pathogen distribution), and the optimal normalized cost is independent of  $\sigma$.   For wide cross-reactivities ($\sigma > \sigma_c$),  the receptors are optimally of a single type with reactivity centered on the pathogen distribution,  while the optimal normalized cost increases with $\sigma$ since the receptor is unnecessarily reactive to  rare pathogens.
  These results arise from a tension between two opposing tendencies.  As in {\TM the case of no cross-reactivity} the statistics of pathogen detection  broaden the optimal receptor distribution relative to the pathogen distribution. 
%  (hence the $(1 + \alpha)$ factor in the variance for the narrow cross-reactivity case). 
   But cross-reactivity has the opposite effect, favoring more concentrated distributions. Here, broadening dominates when cross-reactivity is sufficiently narrow compared to  the pathogen distribution, and concentration dominates  when cross-reactivity is broader.
}


{\VB Does cross-reactivity generically drive the optimal receptor distribution to cluster into peaks?  We investigated
 this question numerically.
For concreteness, consider a linear cost $F(m) = m$, and random pathogen environments in one or two dimensions constructed by drawing $\log Q_a$ independently for each $a$ from a normal distribution, and then normalizing so that $\sum_a Q_a = 1$.  (We distribute the $\log$ of $Q_a$, rather than $Q_a$ itself, to ensure that $Q_a > 0$.)
 For numerical purposes, shape space is taken to be bounded and discretized, and we use  accelerated gradient projection optimisation (\ifthenelse{\equal{\ispnas}{true}}{SI Sec. E}{App.~\ref{app:numerics}}). We find that the optimal repertoire $P^*$ is strongly peaked on a discrete forest of receptors  (Fig.~\ref{fig:crossreactivity}A,B).    However, the peaks are spaced  evenly, at  roughly
% the even spacing of the peaks, with an inter-peak distance of order 
the cross-reactivity scale $\sigma$, suggesting that $P^*$ is smooth when viewed at scales larger than $\sigma$.  Indeed, we  expect that when viewed coarsely, cross-reactivity should be irrelevant and $P^*$ should tend to the solutions in {\TM the previous section} and Table~\ref{tab:costinfluence}.  
}

{\TM Make a reference to \ifthenelse{\equal{\ispnas}{true}}{SI Fig.~S1}{Fig.~\ref{fig:dirac}}}.

\ifthenelse{\equal{\format}{pnasfigend}}{}{\panelthree}

{\VB How can we quantitatively understand such distributions which are fragmentary in detail, but may show organization when viewed coarsely (Fig.~\ref{fig:crossreactivity}B)?   A useful technique, borrowed from work on disordered systems, is to measure the {\em radial distribution function}  \cite{ChaikinLubensky}:
\begin{equation} \label{eq:rdf}
    g(R) = \av{P(r) P(r')}_{|r - r'|=R}
\end{equation}
{\TM where $|r-r'|$ is the distance between points $r$ and $r'$.}
Fig.~\ref{fig:crossreactivity}C presents $g(R)$ for $P^*$ in two dimensions. The initial drop at small $r$ indicates that peaks in $P^*$ are rarely close -- i.e., peaks in the optimal repertoire tend to repel each other.
%there is little chance to find two peaks close to each other, {\TM meaning that peaks tend to repel each other}.
This exclusion, which operates over the range of strong cross-reactivity, is a sensible way to distribute resources, as it limits redundant protection against the same pathogens.
%The effective repulsion occurs over a range of order the cross-reactivity
%The range of distances over which this effective repulsion occurs is of the order of $\sigma$, in line with this argument. 



\todo{The rough periodicity of the peaks in $g(R)$ suggests a tiling property, confirms  even spacing.  The damping indicates disorder.  NOT FINISHED EDITING FROM HERE TO THE END OF THIS SUBSECTION.}


{\TM This allows us to draw an analogy with the problem of sphere packing. When brought to very high densities, hard spheres must cover as much space as possible while maintaining an exclusion zone with other spheres. Our optimisation problem solves a similar problem. When the density becomes very high, packed spheres organise into a disordered tiling pattern, evidenced by damped oscillations in $g(R)$, similar to what we observe. Such a tiling ensures a regular distribution of receptors and a uniform coverage of the antigenic space.
}
}

%The position of the peaks is not random but shows a {\it tiled} structure, which is best seen in the 2D example (Fig. \ref{fig:crossreactivity}B).
%To analyze this structure quantitatively, we use a {\TM measure commonly used in condensed matter physics to describe the arrangement of molecules in liquids, cristals, glass or packing of spheres ---\,the radial distribution function, which measures correlation between peak positions \cite{ChaikinLubensky}:}
%\begin{equation} \label{eq:rdf}
%    g(r) = \av{P(r_1) P(r_2)}_{|r_1 - r_2|=r}
%\end{equation}
%{\TM where $|r_1-r_2|$ is the distance between $r_1$ and $r_2$.}
%Fig.~\ref{fig:crossreactivityanalysis}A represents $g(r)$ for the 2D tiling. {\TM The initial drop at small $r$ indicates that}
%there is little chance to find two peaks close to each other, {\TM meaning that peaks tend to repel each other}.
%This exclusion is a sensible way to distribute resources, as it tends to limit redundant protection of the same region.
%The range of distances over which this effective repulsion occurs is of the order of $\sigma$, in line with this argument. {\TM This allows us to draw an analogy with the problem of sphere packing. When brought to very high densities, hard spheres must cover as much space as possible while maintaining an exclusion zone with other spheres. Our optimisation problem solves a similar problem. When the density becomes very high, packed spheres organise into a disordered tiling pattern, evidenced by damped oscillations in $g(r)$, similar to what we observe. Such a tiling ensures a regular distribution of receptors and a uniform coverage of the antigenic space.
%}

{\TM To quantify how regular the tiling is}, we calculated {\TM the normalized power spectral density} of the 2D pattern. 
%{\TM Assuming that $P(r)$ can be written as a sum of $n$ Dirac deltas, $P(r)=\sum_{i=1}^n p_i\delta(r-r_i)$, 
{\TM We define this spectral density as:}
%\begin{equation} \label{eq:sq}
%    S(q) = \av{\frac{|FT P(r)|^2}{\int \ud r P(r)^2}},
%\end{equation}
\begin{equation}\label{eq:sq}
S(q)=\frac{\sum_{r,r'} P_rP_{r'} e^{{\rm i} q(r-r')}}{\sum_r P_r^2},
\end{equation}
{\TM where $q$  is the wave vector. The normalization is chosen such that, when $P_r$ is made of peaks of uniform heights, $S(q)$ coincides with the {\em structure factor} familiar in condensed matter physics, which satisfies
$S(q \rightarrow \infty) = 1$. Fig.~\ref{fig:crossreactivity}D shows $S(q)$ averaged over many realizations, and over all directions of $q$ so that it only depends on its modulus $|q|$.}
{\TM As expected}, $S(q)$ approaches 1 for large $q$, reflecting the randomness of the precise position of the peaks locally. {\TM (The small departure from $1$ is attributable to the form factor of the peaks, which results from the discretization procedure.)}
$S(q)$ is very low for small $q$, indicating that fluctuations in the number of receptors per surface area are small at large scales. {\TM In other words, the number of receptors contained in a large given area of the shape space is very reproducible. This phenomenon, called {\em hyperuniforminity} in condensed matter \cite{stillinger-2003}, is linked to the incompressibility of the material, and characteristic of jammed packings \cite{Donev:2005p13220,Berthier:2011p13219}.
}
%The structure factor 

%This  behaviour is similar to that predicted for a solid.
{\TM This hyperuniforminity} provides insight into how space is covered {\TM in the optimal solution}:
at large scales (small $q$) the fluctuations in the number of receptors should be suppressed to cover the space more or less uniformly, whereas 
the small scale fluctuations (large $q$) get smoothed out by cross-reactivity and can be tolerated.
{\TM At large scales (small $q$), the fluctuations in the optimal receptor distribution are entirely driven by those of the antigenic landscape (see \ifthenelse{\equal{\ispnas}{true}}{SI Fig.~S2}{Fig.~\ref{fig:kappascaling}}).
%, modulated by the cross-reactivity function $f$.
%At these large scales, the power spectrum of the receptor distribution is approximately given by:
%$|\sum_r P_r e^{\mathrm{i}qr}|^2\sim \kappa^2 \exp[(q\sigma)^2/2]/4$, where $\kappa$ is magnitude of fluctuations in $Q$, and the exponential term stems from the inverse of the Fourier transform of $f$ (see Appendix). We check this relation by plotting the power spectral density normalized by $\kappa^2$
%(Fig.~\ref{fig:crossreactivityanalysis}C), and verify that all curves collapse onto the theoretical prediction $\exp[(q\sigma)^2/2]/4$.
}
%We furthermore see that the fluctuations for small $q$ are purely driven by antigen fluctuations, as seen from the rescaled structure factor that follows exactly the spectral components of the antigen distribution (black line).
%{\color{red} [TM- use the word tiling somewhere?]}
%the fluctuations follows directly the antigen distribution in magnified form (cross-reactivity smoothens!) up to a certain q. {\color{red} ????} 

\ifthenelse{\equal{\format}{pnasfigend}}{}{\panelfour}


{\TM 
So far our analysis has focused on particular choices of the antigenic environment (random white noise), and the cross-reactivity kernel $f$ (Gaussian). To test the generality of our results}, we investigated whether strongly peaked repertoires
were also optimal {\TM in other conditions}. We find that the choice of the cross-reactivity function can qualitatively impact the optimal repertoire. As shown in \ifthenelse{\equal{\ispnas}{true}}{SI Fig.~S3}{Fig.~\ref{fig:kernels}}, changing the cross-reactivity function does not
change the peaked nature of the optimal repertoire, but it does change number and position of the peaks. 
%The antigen distribution we obtain by drawing a number of independent
%random numbers is uncorrelated.
%As antigens mutate, on short timescales the distribution may be correlated, as we have assumed in the analytical example. 
{\TM To account for possible correlations in the distribution of antigens across the effective shape space (reflecting {\em e.g.} phylogenic correlations between pathogens),}
we also generated random correlated antigen distributions by filtering white noise.
In this case we find peaked optimal receptor distributions (Fig. \ifthenelse{\equal{\ispnas}{true}}{SI Fig.~S4}{\ref{fig:correlation}}), similarly to those described above for the uncorrelated antigen distribution. %, characteristic of long timescales.
%{\color{red} Aleks says $\to$ Appendix: 
%If the Fourier transform of the kernel has zero crossings, we can have
%non-uniform optimal solutions even for completely uniform antigen
%distributions.
%The Gaussian kernel we have considered so far, might be considered
%marginal between kernels with and without zero crossings
%\citep{hernandez-garcia-2007}.
%Consider the family of Kernel functions
%$\exp\((-\frac{1}{2}\((\frac{x}{\sigma}\))^\gamma\))$, which includes
%the Gaussian as a special case for $\gamma = 2$.
%Up to $\gamma = 2$ all such Kernels have positive Fourier transforms,
%whereas for $\gamma > 2$ the Fourier transforms take negative values
%\citep{hernandez-garcia-2007}.}
%As shown in Fig. \ref{fig:kernels} changing of the cross-reactivity function does not change the peaked nature of the optimal repertoire, but it does change number and position of peaks.
{\TM The shape space of receptors and antigens is probably highly dimensional, some authors estimating as many as five effective dimensions \cite{oster-1979}.
Although our analysis is here restricted to two dimensions for computational reasons, previous work on the dimensional dependence of random packing problems in physics allows us to
expect all these results to hold more generally in higher dimensions.}


%{\color{red} add paragraph about how the results do not depend on choice of pathogen correlation functions and different kernel choices with ref to fig in SI/appendix.}

%In exploring the effect of cross-reactivity we have made considerable simplifications.
%A word of caution is thus in order, but making strong assumptions allowed us to derive interesting results and get an intuition for the problem.
%A mathematical argument suggests, that the peakedness of solutions in presence of cross-reactivity holds relatively generally (see App. \ref{app:mathpeaks}), but future work should check this conclusion numerically and also carefully investigate whether the other conclusions also hold more generally.




\begin{enumerate}
\item Bottom line -- small scale forest, large scale smoothness reproducing previous section
\item Slightly different pathogen distributions give totally different receptor distributions, but  with similar coverage. Prediction.
\end{enumerate}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Previous Version
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
%\begin{figure}
%    \centering
%    \includegraphics{fig/crossreactivityanalytical}
%    \caption{
%        {\TM Optimal receptor distribution and cost for protecting against
%a one-dimensional Gaussian antigenic landscape $Q(a)$ of variance $\sigma_Q^2$,}
%%an analytically solvable example,
%as a function of the cross-reactivity width $\sigma$.
%{\TM As the $\sigma$ increases, the optimal distribution $P^*(r)$ becomes narrower and narrower (left and middle insets), until it concentrates entirely onto a single point, for $\sigma\geq \sqrt{2}\sigma_Q$ (right inset).
%        The minimal cost (normalized by $\sigma$ for a comparison at constant recognition capability) 
%is constant below the transition point, but increases with $\sigma$ past it.
%%        The antigen distribution $Q(a)$ is Gaussian.
%Here the cross-reactivity kernel, which quantifies the affinity between receptor $r$ and antigen $a$ as a function of their distance in shape space, is assumed to have a Gaussian form:
%        %We assume furthermore that cross-reactivity can be described by a Gaussian kernel
%        $f(r-a) = \exp[-(r-a)^2 / 2\sigma^2]$,
%       and the cost function is linear in the effective recognition time, $F(m) = m$.}
%% first remains constant, before starting to increase for $\sigma>\sqrt{2}\sigma_Q$.
%%        Insets show the pathogen distribution $Q(a)$ and the optimal receptor distribution $P^\star(r)$ for three choices of $\sigma/\sigma_Q$ on both sides of the transition. The optimal receptor distribution becomes narrower as the cross-reactivity width is increased, until it becomes a Dirac delta function at the transition.
%}
%    \label{fig:crossreactivityanalytical}
%\end{figure}
%
%
%\begin{figure}
%    \centering
%    \includegraphics{fig/crossreactivity}
%    \caption{Cross-reactivity plays an important role in shaping the optimal repertoire, often leading to highly peaked repertoires.        
%\TM
%%        (A)-(B) Results from numerical optimization for random antigen landscapes generated according to $Q \propto \ln \mathcal{N}(\kappa)$.
%        The optimal receptor distribution $P^*(r)$ is represented for (A) one- and (B) two-dimensional random environments.
%{\TM
%Despite being peaked, the optimal distribution of receptors covers the antigenic space fairly uniformly, as shown by its coverage by the receptors, $\tilde P^*(a)=\int dr f(a-r)P^*(r)$, represented in the one-dimensional case (A).}
%As in Fig.~\ref{fig:crossreactivityanalytical}, the cross-reactivity kernel is assumed to be Gaussian,
%        %$f(r-p) = \exp\((-\frac{|r-p|^2}{2\sigma^2}\))$
%        $f(r-p) = \exp[-(r-p)^2 / 2\sigma^2]$,
%        and the effective cost function to be linear, $F(m) = m$.
%        {\TM The antigenic landscape $Q(a)$ is generated randomly as the exponential of a Gaussian white noise of amplitude $\kappa=1$. The numerical problem was solved with a discretization step of $0.1\sigma$.}
%%        (A) Exemplary cutout of an optimal receptor distribution.
% %       A one dimensional receptor -- antigen space with periodic boundary conditions is used.
%%        The problem is discretized on a $10\sigma$ grid with a discretization spacing of $0.1\sigma$. 
%%        Due to cross-reactivity the space is still covered fairly uniformly by this collection of peaks. 
%%as shown by the coverage $\tilde P^\star$.
%        %$\kappa = 1$ is used.
%        %(c) Mean spacing between peaks in the optimal receptor distributions increases with $\sigma$.
%        %The slope of the linear regression line is $\sim 1.6$.
%%        (B) Two dimensional receptor -- antigen space with periodic boundary conditions.
%%        The problem is discretized on a $30\sigma \times 30\sigma$ grid with a discretization spacing of $0.1\sigma$.
% %       (C) Exemplary cutout of an optimal receptor distribution for $\kappa = 1$.        
%    }
%    \label{fig:crossreactivity}
%\end{figure}
%
%\begin{figure*}
%    \centering
%    \includegraphics{fig/crossreactivityanalysis}
%    \caption{
%{\TM Structural analysis of the tiling pattern formed by the peaks of the optimal distribution of receptors $P^*(r)$, in two dimensions (see also Fig.~\ref{fig:crossreactivity}B).
%        (A) The radial distribution function of $P^*(r)$ (defined by Eq.~\ref{eq:rdf}) shows a exclusion zone around each peak, followed by oscillations characteristic of a local tiling pattern.
%        (B) Normalized power spectral density $S(q)$ of $P^*(r)$ (defined by Eq.~\ref{eq:sq}) for different values of the parameter $\kappa$ quantifying the heterogeneity of the antigenic lanscape. The high suppression of fluctuations at large scales (small $q$) indicates that the pattern has very little fluctuations in the number of receptors used to cover equal surface areas.
%        (C) The power spectral density of $P^*(r)$, now normalized by $\kappa^2$, shows that the fluctuations at large scale are entirely attributable to those of the antigenic environment, and scale with them, as demonstrated by the data collapse.}
%        The results in (A) and (B) are averaged over 10 independent runs to reduce stochastic fluctuations.
%%        \todo{The values here do not correspond to those used in the simulations. Need to do the simulations.}
%    }
%    \label{fig:crossreactivityanalysis}
%\end{figure*}
%
%In the absence of cross-reactivity, the immune system must have receptors against every possible antigen for full protection, {\TM as discussed in the previous section. Cross-reactivity, the ability of receptors to bind to a variety of different antigens, should in principle allow for a more parsimonious use of receptors to cover the whole range of possible threats. Indeed we will show that, in many cases, the optimal solution concentrates its resources on a few receptors, which together tile the antigenic space.}
%%In the presence of cross-reactivity this is no longer the case.
%
%%We now explore how to optimally introduce receptor cross-reactivity to focus resources on where they are most needed.
%
%Following Perelson and Oster \cite{oster-1979},  we can think of receptors and antigens as points in a common highly dimensional {\it shape space}, whose coordinates can be associated with unspecified physicochemical properties. For simplicity we assume %that the antigen and receptor space can be identified with each other and that 
%the cross-reactivity only depends on the relative position of receptor and antigen in shape space $f_{r,a} = f(r-a)$,  {\TM where $f$ is a decreasing function of the distance between $a$ and $r$.}
%Short distances in shape space correspond {\TM to a good fit between the two molecules, leading to} strong recognition, while large distances translate into weak interactions and poor recognition.%{\color{red} [TM- we haven't said what space we're in, so this is a big ambiguous. from here on we need to introduce the notion of shape space and cite Perelson et al.]}
%
%In order to build some intuition about the problem, we first consider an analytically solvable example, in which the space of receptors and antigens is described by a single continuous number.
%{\TM We assume that the antigen distribution is Gaussian of variance $\sigma_Q^2$, and that the  cross-reactivity function also has a Gaussian form: $f(x)=\exp(-x^2/2\sigma^2)$, where $\sigma$ is the cross-reactivity width, {\em i.e.} the typical distance within which a receptor and an antigen interact.
%The total recognition capability, $\int dx f(x)=\sqrt{2\pi}\sigma$, increases linearly with $\sigma$. Therefore, to make fair comparisons between different values of $\sigma$, we will normalize the overall cost by $\sigma$.}
%%We compare costs at constant total capacity of recognition, i.e. we normalize $f_{r,a}$.
%
%For costs {\TM of the form} $F(m) = m^\alpha$, we can derive the optimal receptor distributions and costs analytically (see App.~\ref{app:gaussian}). 
%The results show two different regimes {\TM depending on the value of the cross-reactivity width $\sigma$}, as illustrated in Fig.~\ref{fig:crossreactivityanalytical}.
%{\TM The optimal normalized cost is constant for narrow cross-reactivities (low $\sigma$), and starts to increase past a critical value $\sigma_c$.
%These two regimes correspond to qualitatively different optimal receptor distributions:
%a Gaussian distribution of variance $(1+\alpha)\sigma_Q^2 - \sigma^2$ below the threshold, and a Dirac delta distribution above it.
%The $1+\alpha$ factor broadens the optimal receptor distribution with respect to the antigen distribution, in accord with the discussion of the previous section, while
%cross-reactivity has the opposite effect, leading to a more concentrated distribution.
%At the critical value $\sigma_c = \sigma_Q\sqrt{1+\alpha} $, the optimal receptor distribution becomes a Dirac delta function, which it remains for $\sigma>\sigma_c$.
%%Since no further narrowing is possible, the distribution remains unchanged as $\sigma$ is increased beyond $\sigma_c$.
%Above the critical $\sigma_c$, the high cross-reactivity means that the system is wasting resources far away from the center of the pathogen distribution, where little antigen threat is present, resulting in an increase of the cost.}
%%the amount of recognition capacity that is unused in the tails of the antigen distribution increases, which explains the increase in the cost function for $\sigma > \sigma_c$.
%
%{\TM How generic is this phenomenon by which the distribution clusters into peaks? To investigate this question we turn to numerical optimisation.}
%%To generalize the result that cross-reactivity %limits local receptor diversity, leading to strongly peaked distributions, holds more generally, 
%%leads to strongly peaked receptor distributions we turn to numerical optimization. %{\color{red} [TM- rewrite sentence]}
%{\TM For concreteness we consider random pathogen environments in one or two dimensions (modeled by a lognormal white noise distribution of antigens) and assume a linear cost function $F(m)=m$.
%For the purpose of the numerics the space is finite and discretized. The optimization problem is solved by an accelerated gradient projection algorithm (App.~\ref{app:numerics}).}
%%For concreteness, we choose a lognormal white noise distribution of antigens \todo{biological motivation} and assume a linear cost $F(m) = m$, but we do not expect these assumptions to qualitatively change our conclusions. \todo{Andreas says: expand in appendix}.
%
%%Generate random numbers from $\ln \mathcal{N}(\kappa) = exp(\kappa Z)$, where $Z$ is a standard normal random variable. Then normalize the distribution.
%%\todo{expand}
%
%
%The numerical results lead to strongly peaked distributions in both one and two dimensions (Fig.~\ref{fig:crossreactivity}A,B), generalizing the observation that cross-reactivity severely limits local receptor diversity.
%{\TM Compared to the Gaussian case discussed earlier, where the antigen distribution only had one scale $\sigma_Q$, here the random antigen distribution includes all possible scales. By analogy with the Gaussian case, we expect the smallest scales to lead Dirac delta peaks. The observed peaks are evenly spaced, with an inter-peak distance of the same order as the cross-reactivity width $\sigma$.}
%%{\TM [don't get this argument]} In the Gaussian case we saw that the variance of the receptor distributions depended on the variance of the antigen distribution relative to the cross-reactivity. In the numerical result, the antigen distribution (blue line in Fig.~\ref{fig:crossreactivity}A) has multiple scales and we {\TM could} expect the receptor distribution to exhibit peaks mirroring the antigen distribution.  %Although the random antigen distribution used in the numerical calculation has features at many scales, whereas the Gaussian distribution in the analytical calculation has only one characteristic scales, both results exhibit a  strongly peaked receptor distributions. {\color{red} [TM- twice the same sentence?]}
%%The spacing of the peaks in the case of the random antigen distribution is similar to the critical cross-reactivity $\sigma_c=\sigma{2}\sigma$ {\TM discussed earlier}.
%%{\TM [TM- does not seem true in 1D]}
%Additionally, the peaks of the receptor distribution approach the limit of Dirac delta functions as the numerical discretization step tends to zero, {\TM suggesting that the true solution is a weighted sum of Dirac deltas} (see Fig.~\ref{fig:dirac}).
%
%The position of the peaks is not random but shows a {\it tiled} structure, which is best seen in the 2D example (Fig. \ref{fig:crossreactivity}B).
%To analyze this structure quantitatively, we use a {\TM measure commonly used in condensed matter physics to describe the arrangement of molecules in liquids, cristals, glass or packing of spheres ---\,the radial distribution function, which measures correlation between peak positions \cite{ChaikinLubensky}:}
%\begin{equation} \label{eq:rdf}
%    g(r) = \av{P(r_1) P(r_2)}_{|r_1 - r_2|=r}
%\end{equation}
%{\TM where $|r_1-r_2|$ is the distance between $r_1$ and $r_2$.}
%Fig.~\ref{fig:crossreactivityanalysis}A represents $g(r)$ for the 2D tiling. {\TM The initial drop at small $r$ indicates that}
%there is little chance to find two peaks close to each other, {\TM meaning that peaks tend to repel each other}.
%This exclusion is a sensible way to distribute resources, as it tends to limit redundant protection of the same region.
%The range of distances over which this effective repulsion occurs is of the order of $\sigma$, in line with this argument. {\TM This allows us to draw an analogy with the problem of sphere packing. When brought to very high densities, hard spheres must cover as much space as possible while maintaining an exclusion zone with other spheres. Our optimisation problem solves a similar problem. When the density becomes very high, packed spheres organise into a disordered tiling pattern, evidenced by damped oscillations in $g(r)$, similar to what we observe. Such a tiling ensures a regular distribution of receptors and a uniform coverage of the antigenic space.
%}
%
%{\TM To quantify how regular the tiling is}, we calculated {\TM the normalized power spectral density} of the 2D pattern. 
%%{\TM Assuming that $P(r)$ can be written as a sum of $n$ Dirac deltas, $P(r)=\sum_{i=1}^n p_i\delta(r-r_i)$, 
%{\TM We define this spectral density as:}
%%\begin{equation} \label{eq:sq}
%%    S(q) = \av{\frac{|FT P(r)|^2}{\int \ud r P(r)^2}},
%%\end{equation}
%\begin{equation}\label{eq:sq}
%S(q)=\frac{\sum_{r,r'} P_rP_{r'} e^{{\rm i} q(r-r')}}{\sum_r P_r^2},
%\end{equation}
%{\TM where $q$  is the wave vector. The normalization is chosen such that, when $P_r$ is made of peaks of uniform heights, $S(q)$ coincides with the {\em structure factor} familiar in condensed matter physics, which satisfies
%$S(q \rightarrow \infty) = 1$. Fig.~\ref{fig:crossreactivityanalysis}B shows $S(q)$ averaged over many realizations, and over all directions of $q$ so that it only depends on its modulus $|q|$.}
%{\TM As expected}, $S(q)$ approaches 1 for large $q$, reflecting the randomness of the precise position of the peaks locally. {\TM (The small departure from $1$ is attributable to the form factor of the peaks, which results from the discretization procedure.)}
%$S(q)$ is very low for small $q$, indicating that fluctuations in the number of receptors per surface area are small at large scales. {\TM In other words, the number of receptors contained in a large given area of the shape space is very reproducible. This phenomenon, called {\em hyperuniforminity} in condensed matter \cite{stillinger-2003}, is linked to the incompressibility of the material, and characteristic of jammed packings \cite{Donev:2005p13220,Berthier:2011p13219}.
%}
%%The structure factor 
%
%%This  behaviour is similar to that predicted for a solid.
%{\TM This hyperuniforminity} provides insight into how space is covered {\TM in the optimal solution}:
%at large scales (small $q$) the fluctuations in the number of receptors should be suppressed to cover the space more or less uniformly, whereas 
%the small scale fluctuations (large $q$) get smoothed out by cross-reactivity and can be tolerated.
%{\TM At small $q$, the fluctuations in the optimal receptor distribution are entirely driven by those of the antigenic landscape, modulated by the cross-reactivity function $f$. At these large scales, the power spectrum of the receptor distribution is approximately given by:
%$|\sum_r P_r e^{\mathrm{i}qr}|^2\sim \kappa^2 \exp[(q\sigma)^2/2]/4$, where $\kappa$ is magnitude of fluctuations in $Q$, and the exponential term stems from the inverse of the Fourier transform of $f$ (see Appendix). We check this relation by plotting the power spectral density normalized by $\kappa^2$
%(Fig.~\ref{fig:crossreactivityanalysis}C), and verify that all curves collapse onto the theoretical prediction $\exp[(q\sigma)^2/2]/4$.
%}
%%We furthermore see that the fluctuations for small $q$ are purely driven by antigen fluctuations, as seen from the rescaled structure factor that follows exactly the spectral components of the antigen distribution (black line).
%%{\color{red} [TM- use the word tiling somewhere?]}
%%the fluctuations follows directly the antigen distribution in magnified form (cross-reactivity smoothens!) up to a certain q. {\color{red} ????} 
%
%
%{\TM 
%So far our analysis has focused on particular choices of the antigenic environment (random white noise), and the cross-reactivity kernel $f$ (Gaussian). To test the generality of our results}, we investigated whether strongly peaked repertoires
%were also optimal {\TM in other conditions}. We find that the choice of the cross-reactivity function can qualitatively impact the optimal repertoire. As shown in Fig.~\ref{fig:kernels}, changing the cross-reactivity function does not
%change the peaked nature of the optimal repertoire, but it does change number and position of the peaks. 
%%The antigen distribution we obtain by drawing a number of independent
%%random numbers is uncorrelated.
%%As antigens mutate, on short timescales the distribution may be correlated, as we have assumed in the analytical example. 
%{\TM To account for possible correlations in the distribution of antigens across the effective shape space (reflecting {\em e.g.} phylogenic correlations between pathogens),}
%we also generated random correlated antigen distributions by filtering white noise.
%In this case we find peaked optimal receptor distributions (Fig. \ref{fig:correlation}), similarly to those described above for the uncorrelated antigen distribution. %, characteristic of long timescales.
%%{\color{red} Aleks says $\to$ Appendix: 
%%If the Fourier transform of the kernel has zero crossings, we can have
%%non-uniform optimal solutions even for completely uniform antigen
%%distributions.
%%The Gaussian kernel we have considered so far, might be considered
%%marginal between kernels with and without zero crossings
%%\citep{hernandez-garcia-2007}.
%%Consider the family of Kernel functions
%%$\exp\((-\frac{1}{2}\((\frac{x}{\sigma}\))^\gamma\))$, which includes
%%the Gaussian as a special case for $\gamma = 2$.
%%Up to $\gamma = 2$ all such Kernels have positive Fourier transforms,
%%whereas for $\gamma > 2$ the Fourier transforms take negative values
%%\citep{hernandez-garcia-2007}.}
%%As shown in Fig. \ref{fig:kernels} changing of the cross-reactivity function does not change the peaked nature of the optimal repertoire, but it does change number and position of peaks.
%{\TM The shape space of receptors and antigens is probably highly dimensional, some authors estimating as many as five effective dimensions \cite{oster-1979}.
%Although our analysis is here restricted to two dimensions for computational reasons, previous work on the dimensional dependence of random packing problems in physics allows us to
%expect all these results to hold more generally in higher dimensions.}
%
%
%%{\color{red} add paragraph about how the results do not depend on choice of pathogen correlation functions and different kernel choices with ref to fig in SI/appendix.}
%
%%In exploring the effect of cross-reactivity we have made considerable simplifications.
%%A word of caution is thus in order, but making strong assumptions allowed us to derive interesting results and get an intuition for the problem.
%%A mathematical argument suggests, that the peakedness of solutions in presence of cross-reactivity holds relatively generally (see App. \ref{app:mathpeaks}), but future work should check this conclusion numerically and also carefully investigate whether the other conclusions also hold more generally.



==> sections/Old/res3.tex <==
% Punchline 3
% - propose population dynamics allowing adaption
% - key ingredient: competition (in line with previous proposals
% - cost function Lyapunov function of corresponding dynamics!
%   --> global convergence
%   --> continually get better even far from the optimum

\subsection{The optimal repertoire can be reached through competition for antigens}
\label{res3}

\begin{figure}
    \centering
    \includegraphics{fig/soo}
    \caption{
A competitive population dynamics scheme allows the population of receptors to adapt to the antigenic environment and self-organize into a state of high protection, {\TM solving the cost minimization problem}.
{\TM The numerical solution of the population dynamics equations (Eq.~\ref{eq:popdyn}) shows the formation of a highly peaked pattern from a uniform initial distribution, as seen from the insets representing $P_r(t)=N_r(t)/\sum_{r'}N_{r'}(t)$.
% {\color{red} whay is top inset. again parameters and all that.}
The top-right inset represents the antigenic environment $Q_a$ driving the dynamics.}
Departure from optimality,  as measured by the relative cost gap {\TM $[\mathrm{Cost} (P_r(t)) - \mathrm{Cost} (P^*_r)]/\mathrm{Cost}(P_r^*)$}, decreases with time and eventually {\TM reaches zero}.
%a repertoire providing optimal protection is reached.
$\sum_r N_r(0) = 10$
\todo{incorporate properly $r = 0.1$, $\gamma_a = 2.0$, lognormal Q with $\sigma = 1$, discretization $\Delta = 0.025$}.
We use $A(x) = 1/(1+x^2)$, $d = 0.01$, $F(m) = m$, $\int f = 1$.
%and solve the ordinary differential equations with a standard solver (ODEPACK's LSODA \cite{hindmarsh-1983}, absolute tolerance $10^{-14}$, relative tolerance $10^{-8}$). details for SI
    }
    \label{fig:soo}
\end{figure}

The results presented so far have established how repertoires should be structured to provide optimal protection.
{\TM Given the global nature of the optimization problem, and the complex interdependences between receptors arising from local and global trade-offs, one could believe that the optimal solution can only be calculated and excecuted through a centralized effector imposing the distribution of resources at the system-wide level.
However such a global, top down organization is impractical in biological systems. 
We will show that the same optimal solution can be reached in a self-organized manner, through 
the competitive evolution of populations of receptors under antigen stimulation. These dynamics only include local interactions between the receptors and the antigens, whose combined effects lead to a solution of the global cost minimization problem defined in the previous sections.
}

%but we have not yet discussed %the processes that can lead to these optimal distributions.
% the question of how to achieve such repertoires in practice.
%We will now investigate the link between self-organized population dynamics of receptor populations %and optimal repertoire distributions.

{\TM We consider a model for the dynamics of receptors that is very similar to that introduced by de Boer, Perelson and collaborators for B and T cells competitive dynamics \cite{perelson-1994,perelson-2001}.}
Its main assumption is that the division of the receptor-expressing lymphocytes is driven by antigen stimulation. Antigens are in limited supply, meaning that
receptors may compete for antigens.
%In order to adapt to the environment, the receptor population dynamics must depend on the encountered antigens.
%We describe this process by a model for the changing repertoire composition in which the receptors that are able to detect the same antigen compete with each other.
The number $N_r$ of receptors of a given type $r$ evolves according to:
\begin{equation} \label{eq:popdyn}
\frac{\ud N_r}{\ud t} = N_r \[[\sum_a Q_a A\((\sum_r N_r f_{r,a}\)) f_{r,a} - d \]]
\end{equation}
Receptors proliferate upon successful recognition, or {\em tickling}, by antigens (first term of the equation) and die with a constant rate $d$ (second term of the equation).
%Receptors get {\it tickled} by the antigens, and
The growth rate of the population of receptors is proportional to the amount of antigens that the receptor can  detect. {\TM In absence of competition, this amount is simply}
 $\sum_a Q_a f_{r,a}$. {\TM But antigen $a$ may bind to other receptors, and its availability for a given receptor will be reduced because of this competitive binding.}
%In the presence of other receptors specific to the same antigen, the growth rate is decreased.
The extent to which an antigen $a$ interacts with the entire pool of receptors is quantified by $\tilde N_a = \sum_r N_r f_{r,a}$. {\TM $\tilde N_a$ can also be viewed} as the {\em coverage} of antigen $a$ by the repertoire.
The availability of antigen $a$ is assumed to be a decreasing function $A(\tilde N_a)$ of its coverage. {\TM The resulting stimulation on $r$ is then modified to: $\sum_a Q_aA(\tilde N_a) f_{r,a}$, thus accounting for the first term in Eq.~\ref{eq:popdyn}.}
%The decrease in growth rate is given by the availability function, $A(\tilde N_a)$, which depends on the the coverage $\tilde N_a$.
%$A(\tilde N_a)$ is generally a decreasing function of $\tilde N_a$.
%The competition for antigen might be a competition for binding, in which an antigen that is bound by one receptor is no longer able to bind to another.
%It might also arise more indirectly, {\em e.g.} from quicker clearing of an infection in the presence of other receptors, that leaves less time for stimulating growth of other receptor populations.
%We take $A(\tilde N_a)=1/(1+N_a^2)$ to saturate for large antigen coverage, following \cite{perelson-2001}.
{\TM For a given pathogenic environment, the total steady-state receptor population size $N_{\infty}$ is set by the death rate $d$, which counter-balances growth at steady state.}


{\TM When the availability function $A$ is precisely matched to the cost function $F(m)$ through the relation}
\begin{equation} \label{eq:condlyapunov}
    A\((\tilde N_a\))=-c'\bar F'\((\tilde N_a/N_{\infty}\))
\end{equation}
(where we recall that Eq.~\ref{eq:avFp} relates $\bar F$ and $F(m)$), the solution to the optimization problem is {\em exactly} realized as a stable fixed point of the dynamics described by Eq.~\ref{eq:popdyn}.
%For a system that fulfills Eq.~\ref{eq:condlyapunov}, a fixed-point analysis shows that a stable fixed point of the dynamics optimizes the associated cost function.
{\TM To understand why this is the case, let us first consider the absence of cross-reactivity. In that case, 
the dynamical equations for each receptor become independent of each other and read: $dN_r/dt=N_r(Q_rA(N_r)-d)$. The availability function now depends on $N_r$, meaning that receptors can only compete with their own kind ---\,they occupy their own antigenic niche. The steady state size of clone $r$ is thus set by the carrying capacity of that niche, $N_r=A^{(-1)}(d/Q_r)$, or zero if that capacity is negative, which is equivalent to Eq.~\ref{eq:bestPr} provided Eq.~\ref{eq:condlyapunov} is satisfied.
A similar argument holds in the presence of cross-reactivity (App.~\ref{app:popdynfixedpoint}).
Cross-reactivity allows for competition across different receptor types, enforcing an effective exclusion between similar receptors, a phenomenon known in ecology as ``competitive exclusion'' \cite{}, and whose relevance for lymphocyte dynamics was already pointed out in \cite{perelson-1994}. This exclusion is the mechanism by which the distribution of receptors clusters into peaks.
Table \ref{tab:costinfluence} shows the availability function $A(\tilde N)$ for several choices of the cost function.
}

{\TM To check that the dynamics actually converge to the optimal solution, we simulated Eq.~\ref{eq:popdyn} numerically for a random antigenic environment in two dimensions, with $A(\tilde N)=1/(1+\tilde N^2)$ [TM- should we rather simulate $A(x)=1/(1+x)^2$, since it's one of the functions we have considered for the cost function? I remember we already discussed this].
Fig.~\ref{fig:soo} shows the dynamics of the receptor distribution $P_r(t)=N_r(t)/\sum_{r'}N_{r'}(t)$, as well as its cost relative to the optimal solution, as a function of time.}
Starting from a uniform initial distribution of receptors, the repertoire %undergoes a pattern formation process, that 
redistributes the receptors into localized peaks.
The peaks become increasingly prominent and well-separated with time, and there are essentially no receptors between the peaks at steady state.
{\TM The cost converges towards the global minimum, indicating that the steady-state solution is indeed optimal.}
{\TM In summary}, the dynamics allow the repertoire to self-organize into a state of high protection.
This observation does not seem to be confined to the specific choice of initial distribution: {\TM a random initial condition converges to the same final repertoire (Fig. \ref{fig:sooapp})}.

%A mathematical fixed-point analysis shows that a stable fixed point of a population dynamics of this type optimizes an associated cost function (App. \ref{app:popdynfixedpoint}).
%The following equation relates cost and availability function:
%\begin{equation} \label{eq:condlyapunov}
%    \bar F'_a\((\tilde P_a\)) = -c A\((\tilde N_a\)),\; c > 0
%\end{equation}
%
%\todo{We note that this condition is only approximately verified in our numerical example.
%The cost function exactly corresponding to the chosen cost function would be somewhat different}
%
In the special case when the the availability function is scale invariant, the equations describing the change in the repertoire composition reduce to the replicator equations \cite{sigmund-1998},
for which we can show that the expected cost is a Lyapunov function of the dynamics (App. \ref{app:popdynlyapunov}).
This observation implies that regardless of the initial condition, the dynamics reaches the fixed point through the continuous descrease of the cost function.

%\todo{Power law unphysical, because A(0) = finite! But nearly true...}


==> sections/significance.tex <==
The adaptive immune system uses the experience of past infections to prepare its limited repertoire of specialized receptors to protect organisms from future threats.  What is the best way of doing this?  Building a theoretical framework from first principles, we predict the composition of receptor repertoires that are optimally adapted to minimize the cost of infections from a given pathogenic environment.   A naive repertoire can reach these optima through a biologically plausible competitive mechanism.  Our findings explain how limited populations of immune receptors can self-organize to provide effective immunity against highly diverse pathogens.  Our results also inform the design and interpretation of experiments surveying immune repertoires.

